Blacklight: Scalable Defense for Neural Networks against Query-Based Black-Box Attacks

Deep learning systems are known to be vulnerable to adversarial examples. In particular, query-based black-box attacks do not require knowledge of the deep learning model, but can compute adversarial examples over the network by submitting queries and inspecting returns. Recent work largely improves the efficiency of those attacks, demonstrating their practicality on today's ML-as-a-service platforms. We propose Blacklight, a new defense against query-based black-box adversarial attacks. The fundamental insight driving our design is that, to compute adversarial examples, these attacks perform iterative optimization over the network, producing image queries highly similar in the input space. Blacklight detects query-based black-box attacks by detecting highly similar queries, using an efficient similarity engine operating on probabilistic content fingerprints. We evaluate Blacklight against eight state-of-the-art attacks, across a variety of models and image classification tasks. Blacklight identifies them all, often after only a handful of queries. By rejecting all detected queries, Blacklight prevents any attack to complete, even when attackers persist to submit queries after account ban or query rejection. Blacklight is also robust against several powerful countermeasures, including an optimal black-box attack that approximates white-box attacks in efficiency. Finally, we illustrate how Blacklight generalizes to other domains like text classification.

==> countermeasure.tex <==

\section{Robustness against Adaptive Attacks}
\label{sec:countermeasure_old}
Any meaningful defense must be robust against adaptive countermeasures from
attackers who understand the defense. We explored a number of customized
adaptive attacks against Blacklight in our work, and present the
strongest attacks here. Two other attacks are summarized in the appendix.
% Next, we consider three
% categories of adaptive adversaries: \textit{skilled adversaries} who try to
% increase the difference between attack queries to bypass detection,
% \textit{smart adversaries} who first try to reverse engineering tracker setting and
% launch attacks based on the reverse engineered knowledge, and \textit{future adversaries}
% who are able to break current constraints for black-box attacks and build stronger attacks.
% We now explore potential countermeasures in these three broad categories.

\begin{table}[t]
  \centering
  \resizebox{.49\textwidth}{!}{
  \begin{tabular}{|l|l|cccc|cccc|}
  \hline
  \multicolumn{2}{|l|}{\multirow{2}{*}{\backslashbox[35mm]{\bf Attack}{\bf Transformation}}} & \multicolumn{4}{c|}{\bf Gaussian Noise w. Different STD} & \multicolumn{4}{c|}{\bf Image Augmentation} \\ \cline{3-10}

    \multicolumn{2}{|l|}{}      &\bf  0.0001    & \bf 0.0005    & \bf 0.005   & \bf 0.05    & \bf Shift   & \bf Rotate   & \bf Zoom   & \bf Comb.  \\ \hline

    \multirow{2}{*}{\bf NES - QL}       & \bf ASR       & 85\%      & 80\%      & 15\%    & 0\%     & 100\%   & 75\%       & 80\%   & 60\%      \\

& \bf ADR                & 100\%     & 100\%     & 100\%   & N/A         & 100\%   & 100\%      & 100\%  & 100\%     \\ \hline
\multirow{2}{*}{\bf NES - LO}                 & \bf ASR                                         & 25\%      & 20\%     & 15\%     & 0\%     & 100\%   & 45\%       & 70\%   & 20\%      \\

&\bf  ADR                & 100\%     & 100\%    & 100\%   & N/A         & 100\%   & 100\%      & 100\%  & 100\%     \\ \hline
  \multirow{2}{*}{\bf Boundary}                         & \bf ASR                                         & 90\%      & 90\%      & 85\%    & 0\%     & 90\%    & 90\%       & 90\%   & 90\%      \\

& \bf ADR                & 100\%     & 100\%     & 100\%   & N/A         & 100\%   & 100\%      & 100\%  & 100\%     \\ \hline
  \multirow{2}{*}{\bf ECO}                              & \bf ASR                                         & 85\%      & 0\%       & 0\%     & 0\%     & 0\%     & 0\%        & 0\%    & 0\%       \\

& \bf ADR                & 100\%     & N/A         & N/A       & N/A         & N/A       & N/A          & N/A      & N/A         \\ \hline
  \multirow{2}{*}{\bf HSJA}                             & \bf ASR                                         & 95\%      & 20\%      &  5\%   & 0\%     &  0\%  &    5\%   &  10\%  &   15\%   \\

&\bf  ADR                & 100\%     & 100\%      & 100\%   & N/A         &  N/A  &     100\%  &    100\% &  100\%   \\ \hline
  \end{tabular}
}
\caption{\small Attack success rate (ASR) and Blacklight attack detection rate (ADR) of successful attacks
  as attackers add different image transformations. Column 3-6 report the results for adding Gaussian Noise with different standard deviation (STD) and Column 7-10
  report the results for applying different image transformations to each attack queries.}
\label{tab:transformation}
\end{table}


\subsection{Attacker-side Countermeasures}

Here we present three adaptive attacks that rely on smarter queries and
attack traffic patterns to evade detection. Two of these are possible today
with general knowledge of Blacklight, and the third is an idealized optimal
attack that assumes the strongest possible black-box attack over the
network.

\para{Evasion via Image Transformations.}  An attacker can try to evade
detection by adding additional perturbations to attack queries, such that it
does not disrupt its iterative optimization process, but is significant
enough to produce differences in query fingerprints between attack queries.
Here we explore 2 types of image transformation.  {\it First}, we consider
adding different magnitudes of Gaussian noise to each attack query. {\it
  Second}, we apply different image augmentation schemes like shift,
rotation, zoom and blending.

Table~\ref{tab:transformation} shows that attack success rate and detection
rate for all the transformations of different attacks on \cifar. For each
image transformation, we show detection success rate on {\em successful
  attacks}. Obviously, sufficiently high noise can disrupt classification
both benign and adversarial.  Blacklight is generally more robust than normal adversarial
examples, {\em e.g.} Blacklight continues to detect attacks at noise levels
where the noise has long since disrupted the attack itself.
For each setting, we run 20 attack traces.  For Gaussian noise, we
add different standard deviations of the Gaussian noise to each
image query from 0.0001 to 0.05 (all inputs normalized to [0,1]).
% Sufficient noise can disrupt the image fingerprint and evade
% detection. However, higher levels of noise make attacks harder
% to converge.
% We stopped at 0.05 since that noise level already disrupts all
% adversarial attacks from functioning.
% ,  with standard deviation % $\geq$ 0.05.
Table~\ref{tab:transformation} shows that as noise levels
increase, attack success rates drop quickly. But at all noise levels,
Blacklight is able to detect all successful attacks. % Thus, Gaussian
% noise has no discernable impact on Blacklight's attack detection.

For image augmentation, we test 4 different cases where the attacker shifts
each query by up to 10\%, rotates inputs by up to $10^{\circ}$, zooms into
each query by up to 10\% and where all three techniques are
combined. Table~\ref{tab:transformation}
shows that while different attacks react differently to image augmentation
techniques (some still produce successful attacks while others fail
completely), Blacklight is able to detect all successful attack traces under
different type of augmentations.

\para{Pause and Resume Attacks.}  Adversaries can try to evade detection by
exploiting the fact that Blacklight periodically resets its database.  They
can pause their attack every time it receives a
rejection response, and resuming the attack the next time Blacklight resets
its database. We run experiments through all 5 black-box attacks using this
strategy against a \cifar{} model and Blacklight. We run 100 instances of
each attack, and show average total queries needed for each attack to
succeed, and the average number of reset cycles that requires in
Table~\ref{table:cycles}.  If we reset Blacklight every 24 hours, the fastest
successful attacker would complete an attack (using HSJA) in $1092$ days or
roughly 3 years. While this strategy does allow for a successful attack, the
time cost to perform this attack makes it highly impractical.

% \subsection{Ideal Adversaries}
% Novel black-box attacks are being proposed at a rapid rate. Many of them
% break current assumptions on what black-box attacks can and cannot do. For
% example, future attacks may allow larger perturbation budgets, or find novel
% methods to dramatically reduce the number of queries necessary to converge to
% an adversarial example. In this section, we hypothesize about potential
% future black-box attacks that break current constraints, and evaluate
% Blacklight against some {\em ideal} black-box attacks.


\begin{table}[t]
  \centering
  \resizebox{.45\textwidth}{!}{
\begin{tabular}{|l|c|c|c|c|}
\hline
\backslashbox{Attack Type}{$N$}       & 500               & 100              & 50               & 10               \\ \hline
NES - Query Limit & 100\%             & 100\%            & 100\%            & 95\%             \\
NES - Label Only  & 100\%             & 100\%            & 100\%            & 31\%             \\
Boundary          & 100\%             & 90\%             & 89\%             & 48\%             \\
ECO               & 100\%             & 100\%            & 100\%            & 100\%            \\
HSJA              & 100\%             & 100\%            & 100\%            & 91\%             \\ \hline
CW                & \multicolumn{4}{l|}{Average $N$ = 6.33, Detection rate = 100\%} \\
PGD               & \multicolumn{4}{l|}{Average $N$ = 3.13, Detection rate = 81\%}  \\ \hline
\end{tabular}}
\caption{\small Blacklight's performance against near-optimal
  ``query-efficient'' and ``perfect-gradient'' black-box attacks.}
\label{table:stronger_attack}
\end{table}

\para{Optimal Black-Box Attacks.} Since black-box network attacks are
continuously evolving in query efficiency, we also evaluate Blacklight
against two types of highly efficient attacks that are possible but do not
yet exist. First, we consider extremely ``query-efficient'' black-box attacks
that require orders of magnitude fewer attack queries than current
attacks. To simulate a near-optimal query-efficient attack, we evenly downsample
attack query traces from our current 5 attacks to generate attack
traces that are a tiny fraction of current traces. We then test Blacklight's
detection performance on these subsampled attack traces.
Table~\ref{table:stronger_attack} shows that even when attacks are able to
complete in 500, 100, or 50 queries, Blacklight still detects them near
perfectly (100\% detection for 4 attacks and 89\% for Boundary attack). Even
when these attacks complete within 10 queries, Blacklight is still highly
successful at detecting NES-QL, ECO and HSJA.

Second, we imagine a ``perfect-gradient'' black-box algorithm that is somehow
able to perfectly predict gradient functions from the results of its attack
queries, as accurately as a white-box attack. Each iteration of the
gradient calculation for an analogous white-box attack would translate to a
single query over the network by the black-box attacker.  This idealized
black-box attack uses CW~\cite{carlini2017towards} and
PGD~\cite{madry2017towards} to generate attack sequences against our \cifar{}
model.  On average, CW and PGD converge after only $6.3$ and $3.1$
queries. Against simulated black-box attacks using these attack queries,
Blacklight detects $100\%$ of attacks driven by CW, and $81\%$ of PGD-driven
attacks.



\subsection{Reverse Engineering Attack}
\label{sec:smart}

Beyond first order adaptive attacks, we worked hard to design more powerful
adversarial attacks specifically targeted against Blacklight. The strongest
attack we could design is the two-pronged reverse engineer attack, where an
attacker first uses queries to probe the limits of a Blacklight system's configuration
parameters, and then leverages those results to optimize a guided
transformation attack.

We consider an attack strategy where adversaries applies two sets of pixel modifications
to an input to some MLaaS model over the network. One set of changes is
applied in order to produce the desired misclassification on the input, and
the other set is applied solely for the purposes of evading Blacklight.
Since Blacklight uses a quantization process to limit the number of hashes
computed, an attacker who knows precisely how quantization is configured can
carefully modify pixels near the boundary, with the net effect of altering
many hash values without changing too many pixels in aggregate (and thus not
altering the input significantly).

find the pixel values near the boundary and make the pixel values change
after quantization by adding very small perturbations to those pixels. They
can choose those pixels as the set to bypass detection and apply customized
image transformation that is able to add the small perturbation to the attack
queries and evade Blacklight's detection. In general, we find that
adversaries can reverse engineer the quantization boundary and achieve
20\%-25\% attack success rate with mitigation when pixel quantization uses
salt $salt_q$ but fail otherwise.
% The key intuition of this countermeasure is to add just enough perturbation to a small set
% of pixels in each window in order to alter the hash.


\para{Inferring Quantization Boundaries.}
First, the adversary needs to obtain quantization step used by the defender. To do so, the adversary send queries to the detection system
with different pairs of images, $(x_i, x_i + K)$, where K is an image with value $k$ for every pixel.
The adversary submits both $x_i$ and $x_i+K$ and if the $x_i+K$ query is
rejected by the system, it means $k$ is smaller than the quantization step used by the defender.
Using a binary search, the adversary can efficiently reverse engineer the value of quantization step
and get the boundaries for quantization. Since a single post-quantization pixel change affects $w/p-1$ continuous hash
values, to change most hash values using fewest pixels, the best strategy is to change one pixel very $D$ pixels.
To estimate $D$, we can send pairs of queries ($x_i, x_i'$) to the detection systems where in $x_i'$ one pixel is
changed after quantization every $D_i$ pixels. If the detection system rejects $x_i'$, then $D_i$ is too large to bypass
detection and it has to be smaller. We keep decreasing $D$ until we find the one can bypass the detection system.


With the knowledge of boundaries for quantization and distance $D$, an adversary can then compute
precisely which pixels to modify so as to alter the maximum number of potential fingerprint hash
values.  The perturbation must be large enough to survive quantization, and each query must choose
its pixel perturbation to produce distinct hashes from that of all prior perturbations.
In order to stay in the attack budget, the attacker identifies the set of pixels that are closest
to the quantization boundary and only perturb these pixels.

We apply the guided transformation attack to the two fastest converging
attacks (ECO and HSJA) and test the attack on Blacklight with mitigation enabled.
The attacker achieves $20\%$ and $25\%$ attack success rate for ECO and HSJA respectively.

\para{Guided transformations with $salt_q$.} The defender can overcome the above adversary by making it
harder to extract quantization boundary. Rather than having the same quantization boundary
for each pixel, the defender can add salt to the process and make the quantization boundary different for each pixel as shown in Equation~\ref{eq:quantization}.
Under such scenario, the adversary's reverse engineering techique cannot extract the per pixel boundary,
because the thresholds for different pixels are not correlated and
the attacker does not know which pixels are attributed to the detection results.

Without the information of quantization boundary, the adversary is still able to
launch a weaker version of their attack by perturbing a larger number of pixels and hope some of
the changes are able to persist through quantization and alter the hashes.
We implement such attack by altering $5$, $10$, and $15$ out of every $20$ pixels within the
perturbation budget. Then we test apply the transformation to ECO and HSJA attack.
Both attacks have $0\%$ attack success rate. Thus, when deploying Blacklight, the quantization
salt is significant to guarantee the security of the system.


\begin{table}[t]
  \centering
  \resizebox{.49\textwidth}{!}{
  \begin{tabular}{@{\extracolsep{1pt}}|l|c|c|}
      \hline
      Attack Type & Average Reset Cycles Needed & Average Total Queries\\
      \hline
      NES-QL & 11471 & 12695 \\
      NES-LO  & 65837 & 67099 \\
      Boundary   & 2285 & 6160 \\
      ECO             & 16590 & 16591 \\
      HSJA            & 1092 & 1121 \\
      \hline
  \end{tabular}}
\caption{Average reset cycles needed for a successful Pause and Resume attack
  on \cifar{}. The fastest attack (HSJA) can succeed in roughly 3 years.}
\label{table:cycles}
\end{table}


==> discuss.tex <==
\vspace{-0.1in}
\section{Discussion}
\vspace{-0.1in}

There exist some variants for black-box adversarial attacks where we have not included
in our evaluation. Suya et. al.~\cite{suya2020hybrid} propose {\em hybrid black-box adversarial attack}
where the attacker first uses substitute model attack to generate adversarial examples
and then uses these adversarial examples as starting points to launch query-based attacks. Since
the hybrid attack still has a query-based attack component, Blacklight can be used to defend against this
type of attacks. Although the authors show that by leveraging hybrid attacks the queries needed drop to
some extent, hundreds or thousands of queries are still needed to launch a successful attack, which
is far larger than the number of queries needed by Blacklight to detect an attack.

{\em Adversarial patch attacks}~\cite{brown2017adversarial, karmon2018lavan},
another variant of adversarial attacks, propose that instead of applying
an imperceptible perturbation to every pixel in the inputs, attackers can add a localized visible perturbation as
a patch on the input to cause misclassifications. Adversarial patches can be both trained for a single image or
multiple images. Recently, Yang et. al.~\cite{yang2020patchattack} have proposed to use reinforcement learning to train single-image based adversarial patches under black-box threat model. For this attack, since the patch size is usually very small and the background is always the same image, most of the
image stays the same in the attack queries. Thus, Blacklight can also be used to defend against single-image based adversarial patch
attacks. For adversarial patches generated to be effective across multiple images, the white-box attack alone takes hundreds to thousands of iterations,
implying that a black-box attack of this type may be computationally infeasible in practice. Thus, although this type of attack could potentially
bypass Blacklight due to the use of different images, we defer its investigation to future work due to the lack of a standardized,
query-efficient method to carry it out.

